Exploring the Solar System with the NOIRLab Source Catalog I: Detecting Objects with CANFind

Despite extensive searches and the relative proximity of solar system objects (SSOS) to Earth, many remain undiscovered and there is still much to learn about their properties and interactions. This work is the first in a series dedicated to detecting and analyzing SSOs in the all-sky NOIRLab Source Catalog (NSC). We search the first data release of the NSC with CANFind, a Computationally Automated NSC tracklet Finder. NSC DR1 contains 34 billion measurements of 2.9 billion unique objects, which CANFind categorizes as belonging to "stationary" (distant stars, galaxies) or moving (SSOs) objects via an iterative clustering method. Detections of stationary bodies for proper motion (mu) less than 2.5"/hr (0.017 degrees/day) are identified and analyzed separately. Remaining detections belonging to hi-mu objects are clustered together over single nights to form "tracklets". Each tracklet contains detections of an individual moving object, and is validated based on spatial linearity and motion through time. Proper motions are then calculated and used to connect tracklets and other unassociated measurements over multiple nights by predicting their locations at common times forming "tracks". This method extracted 527,055 tracklets from NSC DR1 in an area covering 29,971 square degrees of the sky. The data show distinct groups of objects with similar observed mu in ecliptic coordinates, namely Main Belt Asteroids, Jupiter Trojans, and Kuiper Belt Objects. Apparent magnitudes range from 10-25 mag in the ugrizY and VR bands. Color-color diagrams show a bimodality of tracklets between primarily carbonaceous and siliceous groups, supporting prior studies.

==> NSC CANFind/authors.tex <==

\correspondingauthor{Katie M. Fasbender}
\email{katiefasbender@montana.edu}

\author[0000-0003-1622-5901]{Katie M. Fasbender}
\affiliation{Department of Physics, Montana State University, P.O. Box 173840, Bozeman, MT 59717-3840}

\author[0000-0002-1793-3689]{David L. Nidever}
\affiliation{Department of Physics, Montana State University, P.O. Box 173840, Bozeman, MT 59717-3840}
\affiliation{NSF's National Optical-Infrared Astronomy Research Laboratory, 950 North Cherry Ave, Tucson, AZ 85719}

\shortauthors{Fasbender et al.}

==> NSC CANFind/shorthand.tex <==
\newcommand{\kms}{\mbox{km s$^{-1}~$}} 
\newcommand{\kmse}{\mbox{km s$^{-1}$}} 
\newcommand{\ms}{\mbox{m s$^{-1}~$}} 
\newcommand{\mse}{\mbox{m s$^{-1}$}} 
\newcommand{\rsun}{R$_{\odot}$} 
\newcommand{\msun}{M$_{\odot}~$} 
\newcommand{\msune}{M$_{\odot}$} 
\newcommand{\vhelio}{$V_{\rm HELIO}~$}
\newcommand{\vhelioe}{$V_{\rm HELIO}$}
\newcommand{\vlsr}{$V_{\rm LSR}~$}
\newcommand{\vlsre}{$V_{\rm LSR}$}
\newcommand{\vlgsr}{$V_{\rm LGSR}~$}
\newcommand{\vgsr}{$V_{\rm GSR}~$}
\newcommand{\vgsre}{$V_{\rm GSR}$}
\newcommand{\lms}{$L_{\rm MS}~$}
\newcommand{\lmse}{$L_{\rm MS}$}
\newcommand{\bms}{$B_{\rm MS}~$}
\newcommand{\bmse}{$B_{\rm MS}$}
\newcommand{\dgr}{$^{\circ}~$}
\newcommand{\vhel}{$V_{\rm HEL}~$}
\newcommand{\vhele}{$V_{\rm HEL}$}
\newcommand{\h}{$^{\rm h}$}
\newcommand{\m}{$^{\rm m}$}
%\newcommand{\s}{$^{\rm s}~$}
\newcommand{\se}{$^{\rm s}$}
\newcommand{\nhi}{$N_{\rm H \small{I}}$ }
\newcommand{\nhie}{$N_{\rm H \small{I}}$}
\newcommand{\pcm}{cm$^{-2}$ }
\newcommand{\pcme}{cm$^{-2}$}
\newcommand{\hi}{H{\footnotesize I} }
\newcommand{\hie}{H{\footnotesize I}}
%\newcommand{\hi}{\ion{H}{1} }
%\newcommand{\hie}{\ion{H}{1}}
\newcommand{\chisq}{$\chi^2$~}
\newcommand{\chisqe}{$\chi^2$}
\newcommand{\rchisq}{$\chi^2_{\nu}$~}
\newcommand{\rchisqe}{$\chi^2_{\nu}$}
\newcommand{\teff}{$\rm T_{eff}$~}
\newcommand{\teffe}{$\rm T_{eff}$}
\newcommand{\logg}{$\log{g}$~}
\newcommand{\logge}{$\log{g}$}
\newcommand{\metal}{[M/H]~}
\newcommand{\metale}{[M/H]}
\newcommand{\vsini}{$v\sin{i}$~}
\newcommand{\vsinie}{$v\sin{i}$}

\newcommand{\arh}{\arcsec hr$^{-1}$}
\newcommand{\ded}{$^{\circ}$day$^{-1}$}

\definecolor{gold}{rgb}{.8,.6,0}
\newcommand{\kt}[1]{\textcolor{gold}{kt:~#1}} 
\newcommand{\dln}[1]{\textcolor{blue}{dln:~#1}}

\newcommand{\package}[1]{\textsl{#1}}

% Edit 1 
%-----------------------------------------------------
%edit (``additional'' by me)
\newcommand{\editone}[1]{\textcolor{red}{\textbf{#1}}} 
\newcommand{\eonesout}[1]{}%{\textcolor{red}{\sout{#1}}}
 %edit (in response to review)
\newcommand{\editonex}[1]{\textcolor{blue}{\textbf{#1}}}
\newcommand{\eonexsout}[1]{\textcolor{blue}{\sout{#1}}}
%edit (final color - black to make them all look same)
\newcommand{\editoneb}[1]{\textcolor{black}{#1}}

% Edit 2
%-----------------------------------------------------
\newcommand{\eone}[1]{\textcolor{red}{\textbf{#1}}}
\newcommand{\etwosout}[1]{}%{\textcolor{red}{\sout{#1}}}
\newcommand{\edittwob}[1]{\textcolor{black}{#1}}


% Edit 3
%-----------------------------------------------------
%\newcommand{\ethree}[1]{\textcolor{red}{\textbf{#1}}}
\newcommand{\ethree}[1]{\textcolor{black}{#1}}
\newcommand{\ethreesout}[1]{}%{\textcolor{red}{\sout{#1}}}
\newcommand{\editthreeb}[1]{\textcolor{black}{\textbf{#1}}}

%\newcommand{\ignore}[1] %how to get stuff in a command to not show up





